DropCluster: A structured dropout for convolutional networks

Dropout as a common regularizer to prevent overfitting in deep neural networks has been less effective in convolutional layers than in fully connected layers. This is because Dropout drops features randomly, without considering local structure. When features are spatially correlated, as in the case of convolutional layers, information from the dropped features can still propagate to subsequent layers via neighboring features. To address this problem, structured forms of Dropout have been proposed. A drawback of these methods is that they do not adapt to the data. In this work, we leverage the structure in the outputs of convolutional layers and introduce a novel structured regularization method named DropCluster. Our approach clusters features in convolutional layers, and drops the resulting clusters randomly during training iterations. Experiments on CIFAR-10/100, SVHN, and APPA-REAL datasets demonstrate that our approach is effective and controls overfitting better than other approaches.

==> table/ablation_table.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     
%                    Table 1
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\begin{table*}[t]
\centering
\begin{tabular}{ccc}
%%%%%%%%%%%%  LeNet5-CIFAR10 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
   \includegraphics[width=\awidf]{dropout-cifar10-lenet5.png} &
   \includegraphics[width=\awidf]{dropblock-cifar10-lenet5.png} &
   \includegraphics[width=\awidf]{dropcluster-cifar10-lenet5.png} \\
(a) Dropout-CIFAR10-LeNet5 &
(b) DropBlock-CIFAR10-LeNet5 &
(c) DropCluster-CIFAR10-LeNet5 \\

% %%%%%%%%%%%%  LeNet5-CIFAR100 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\includegraphics[width=\awidf]{dropout-cifar100-lenet5.png} &
\includegraphics[width=\awidf]{dropblock-cifar100-lenet5.png} &
\includegraphics[width=\awidf]{dropcluster-cifar100-lenet5.png} \\
(d) Dropout-CIFAR100-LeNet5 &
(e) DropBlock-CIFAR100-LeNet5 &
(f) DropCluster-CIFAR100-LeNet5\\

% %%%%%%%%%%%%  AlexNet-CIFAR100 %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\includegraphics[width=\awidf]{dropout-cifar100-alexnet.png} &
\includegraphics[width=\awidf]{dropblock-cifar100-alexnet.png} &
\includegraphics[width=\awidf]{dropcluster-cifar100-alexnet.png} \\
(g) Dropout-CIFAR100-AlexNet &
(h) DropBlock-CIFAR100-AlexNet &
(i) DropCluster-CIFAR100-AlexNet

\end{tabular}
\caption{Ablation study on CIFAR-10/100 datasets.}
\label{fig:ablation_cifar}
\end{table*}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%     
%                    Table 2
%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


\begin{table*}[h]
\centering
\begin{tabular}{ccc}
%%%%%%%%%%%%  LeNet5-SVHN %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
 \includegraphics[width=\awidf]{dropout-svhn-lenet5.png} &
\includegraphics[width=\awidf]{dropblock-svhn-lenet5.png} &
\includegraphics[width=\awidf]{dropcluster-svhn-lenet5.png} \\
(a) Dropout-SVHN-LeNet5 &
(b) DropBlock-SVHN-LeNet5 &
(c) DropCluster-SVHN-LeNet5 \\

% %%%%%%%%%%%%  LeNet5-AGE-CLF %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\includegraphics[width=\awidf]{dropout-age-clf-lenet5.png} &
\includegraphics[width=\awidf]{dropblock-age-clf-lenet5.png} &
\includegraphics[width=\awidf]{dropcluster-age-clf-lenet5.png} \\
(d) Dropout-APPA-CLF-LeNet5 &
(e) DropBlock-APPA-CLF-LeNet5 &
(f) DropCluster-APPA-CLF-LeNet5\\

% %%%%%%%%%%%%  LeNet5-AGE-RGE %%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\includegraphics[width=\awidf]{dropout-age-rg-lenet5.png} &
\includegraphics[width=\awidf]{dropblock-age-rg-lenet5.png} &
\includegraphics[width=\awidf]{dropcluster-age-rg-lenet5.png} \\
(g) Dropout-APPA-REG-LeNet5 &
(h) DropBlock-APPA-REG-LeNet5 &
(i) DropCluster-APPA-REG-LeNet5

\end{tabular}
\caption{Ablation study on SVNH and APPA-REAL datasets.}
\label{fig:ablation_svnh_age}
\end{table*}

==> table/acc_tab.tex <==

\begin{table}[hb]
\small
\centering
\caption{Classification Accuracy of LeNet-5 train on CIFAR-10 datasets with different dropout types.}
\vskip 0.15in
\adjustbox{width=0.7\textwidth}{
\label{tab:exp_accuracy}
	\begin{tabular}{lcccccc}
		\toprule
		& \multicolumn{3}{c}{\textbf{Acc@1}} 
            & \multicolumn{3}{c}{\textbf{Acc@5}} \\
		\cmidrule(r){2-7}
		 & \textbf{Train}
            & \textbf{Test} 
		 & \textbf{Std} 
           & \textbf{Train}
            & \textbf{Test} 
		 & \textbf{Std}  \\
		\midrule
		No-drop & 99.816 & 60.891	
		        & \colorbox{red!25}{0.461} 
                    & 99.997 
                    & 94.970	
		        & \colorbox{yellow!25}{0.221}\\
		Dropout &  76.477 
                    & \colorbox{yellow!25}{67.389}	
		        & 0.954	 
                    & 98.783 
                    & \colorbox{yellow!25}{96.776}
		        & 0.290\\
		DropBlock & 75.748 & 66.229	
		          & 1.135	
                    & 98.634 & 96.437	
		          & 0.387\\
		DropCluster & 69.239 
                        & \colorbox{red!25}{68.213}	
		            & \colorbox{yellow!25}{0.530} 
                        & 97.637 
                        & \colorbox{red!25}{97.123}	
		              & \colorbox{red!25}{0.190}\\	
		 \bottomrule
	\end{tabular}
 }
\end{table}

==> table/table.tex <==

\begin{table}[htb]
\caption{Comparison of dropout types on LeNet-5 and AlexNet (only when noted). We compute the Cross-Entropy loss for the four classification tasks on the left, and the $L_1$ loss for the rightmost regression task. We report average loss values and corresponding standard deviations after 10 runs.
	}
\label{tab:exp_result}
\vskip 0.15in
\centering
\adjustbox{width=0.9\textwidth}{
	\begin{tabular}[width=\columnwidth]{lccccccccc}
		\toprule
		& \multicolumn{3}{c}{CIFAR-10} 
		& \multicolumn{3}{c}{CIFAR-100} 
            & \multicolumn{3}{c}{CIFAR-100-AlexNet} \\
		\cmidrule(r){2-10}
		 & \textbf{Train}  &\textbf{Test} & \textbf{Std} 
		 & \textbf{Train}  &\textbf{Test} & \textbf{Std}
          & \textbf{Train}  &\textbf{Test} & \textbf{Std} \\
		
		\midrule
		No-drop & 0.865	& 1.084	& \colorbox{red!25}{0.014}
		        &1.614	& 3.293 & 0.152  
                    &0.308	& 5.020	& 0.633  \\
		Dropout &  0.647 &\colorbox{yellow!25}{0.980} &0.034	
		        &2.163	&2.737	&0.036 
                    &1.388	&\colorbox{yellow!25}{2.347}	&\colorbox{yellow!25}{0.036} \\
		DropBlock & 0.686 &1.040 &0.080	
		         &2.399	&2.716	& \colorbox{red!25}{0.028}	
                   &1.638	&2.419	&0.048    \\
		DropCluster & 0.868	&\colorbox{red!25}{0.915}	&\colorbox{yellow!25}{0.017}
		            &2.276	&\colorbox{red!25}{2.657}	&\colorbox{yellow!25}{0.029}	
                        &1.983	&\colorbox{red!25}{2.228}	& \colorbox{red!25}{0.016}  \\		           
        \midrule
            & \multicolumn{3}{c}{SVHN}
		&  \multicolumn{3}{c}{APPA-REAL-CLF} 
		& \multicolumn{3}{c}{APPA-REAL-REG} \\
		\cmidrule(r){2-10}
            & \textbf{Train}  &\textbf{Test} & \textbf{Std}
		  & \textbf{Train}  &\textbf{Test} & \textbf{Std}
		  & \textbf{Train}  &\textbf{Test} & \textbf{Std} \\
		  \midrule
		No-drop   &0.187	&0.480	&0.026
                     &0.104	&12.743	&1.184	
		        &0.305	&10.200	&\colorbox{yellow!25}{0.158}  \\
		Dropout  &0.335	&0.385	&0.016
                    &1.255	&\colorbox{yellow!25}{2.516}	&\colorbox{yellow!25}{0.119}	
		        &1.397	&\colorbox{yellow!25}{10.025}	&0.169 \\
		DropBlock &0.379	&\colorbox{yellow!25}{0.383}	&\colorbox{yellow!25}{0.013}
                  &1.357	&2.597	&0.129	
		         &1.867	&10.283	&0.172 \\
		DropCluster &0.339	& \colorbox{red!25}{0.358} &\colorbox{red!25}{0.007}
                        &1.813	&\colorbox{red!25}{2.346}	&\colorbox{red!25}{0.025}	
		            &2.063	&\colorbox{red!25}{9.976}	&\colorbox{red!25}{0.154} \\
		 \bottomrule
	\end{tabular}
 }
\end{table}
